A Metric for Evaluating and Comparing Closed-Loop Deep Brain Stimulation Algorithms

Objective: Closed-loop deep brain stimulation (DBS) may improve current clinical DBS treatment for neurological movement disorders, but control algorithms may perform differently across patients. New metrics are needed for comparing and evaluating closed-loop algorithm performance that address the specific needs of closed-loop neuromodulation controllers. Approach: A metric is proposed for system performance that includes normalized terms that can be used to compare algorithm performance for a patient. This metric was evaluated using two closed-loop control algorithms that were tested in patients with Parkinson's Disease (PD) who experience rest tremor. Main Results: The metric's resulting balance between tremor treatment and power savings varied on a per patient and algorithm basis. This was expected given how each trial resulted in a variable reduction in stimulation power at the cost of additional tremor for the patient when compared to open-loop stimulation. Significance: The proposed metric will aid in clinical evaluation of new algorithms and provide a benchmark for future system designers. This will be important given the growing potential applications of dynamically adjusted neural stimulation. ClinicalTrials.gov Identifier: NCT02384421.

==> prior versions/introduction_premerge.tex <==
\section{Introduction}\label{sec:Introdcution}
% Overview of current DBS usage
Deep brain stimulation (DBS) refers to the use of electrical stimulation to modulate neural activity far beneath the surface of the brain. Over the last decade, deep brain stimulation (DBS) has rapidly become an important tool in the treatment of a variety of neurological disorders. DBS has proven to be a safe and effective clinical method of treating Parkinson's disease\cite{deuschl2006PDrandomized}, essential tremor\cite{sydow2003multicentre}\cite{flora2010dbs_et}, and dystonia\cite{vidailhet2005bilateral}. When pharmacological methods are not sufficient to dampen the worsening symptoms in these progressive neurological movement disorders, DBS is used as a last resort as it requires brain surgery \cite{gironell2009review}.

% Overview of current problems with DBS
While DBS devices can have a dramatic positive impact on the symptoms of patients with neurological movement disorders, there is considerable room for improvement in the current clinically deployed systems. For instance, the stimulation of brain tissue can cause a variety of unintended side effects \cite{kuncel2006clinical}. Also the power requirements of the stimulation are the largest factor in the decreased overall expected lifetime of the device. When the battery is depleted, surgery is required to replace the pulse generator. It is also difficult for the clinician to select effective stimulation parameters \cite{kuncel2006clinical}. Additionally, even when effective parameters are chosen, many neurological movement disorders are quite variable or intermittent, hence constant stimulation may waste battery life. A pressing issue regarding deep brain stimulation can be stated as follows: existing DBS systems do not take into account the variable nature of neurological movement disorders \cite{hebb2014creating_fb}. Instead these systems simply stimulate deep brain structures at a constant level and consistent rate.

% Proposed solution
A proposed solution to address this problem is to create a feedback loop where DBS parameters are adjusted based on the severity of symptoms that a patient experiences in `real time'. This requires the development and exploration of sensors and classification algorithms that can recognize and measure symptom states. It also requires systems with the ability to communicate with and update the stimulation parameters in an implanted neurostimulator.

% Paper Introduction
In this paper, we present a closed-loop DBS system capable of using wearable sensors that can sense tremor and respond by adjusting stimulation parameters of an implanted DBS device. The feasibility of this system is demonstrated with the cooperation of patients with rest tremor from Parkinson's Disease. In our work, tremor is estimated through the use of inertial measurements taken from worn miniaturized accelerometers and gyroscopes that are mounted in a smart-watch. These tremor estimates are used to calculate updated stimulation amplitudes, which are then transmitted to an implanted Activa PC+S neurostimulator using the Nexus-D communication system by our custom software. As a preliminary demonstration of the wearable closed-loop DBS system, we present the results of several example control paradigms tested with our patients. The purpose of these tests is to demonstrate the real-time system's ability to respond to sensed limb tremor and record the patient's response to the stimulation. Finally, we conclude with a discussion of the ability of these systems to capture data that will be useful to further enhance clinical treatment options and advance our scientific understanding of the underlying neurological mechanisms that produce movement disorder symptoms.
